Thermal Generation of Spin Current in a Quantum Dot Coupled to Magnetic Insulators

In this work, we study thermally-generated spin current in the system consisting of a quantum dot connected to two magnetic insulators. The external leads are kept at different temperatures which leads to an imbalance of magnon populations in two magnetic insulators resulting in the flow of the magnon (spin) current. We take into account many-body magnon interactions and incorporate energy-dependent density of states of the magnetic insulators. Both features can strongly affect magnon distribution in the magnetic insulators and the coupling strengths between the leads and the dot, and thus, the thermally generated spin current. All the calculations are carried out in the weak coupling regime. We show, that results obtained with a density of states being a function of energy differ significantly from the ones obtained with a density of states taken as a constant. In turn, magnon interactions in the leads proved to be important at high temperatures and large values of energy of transported spin waves.

==> Sections/Abstract.tex <==
%Spin caloritronics aims to study the thermal generation and conversion of spin current. %Systems containing quantum dots are especially promising for thermogeneration. In the case of %spin current carried by quanta of spin waves energy-dependent density of states and many-%body interactions are important factors which may affect transport properties in a %meaningful in the right conditions. 
In this work, we study thermally-generated spin current in the system consisting of a quantum dot connected to two magnetic insulators. The external leads are kept at different temperatures which leads to an imbalance of magnon populations in two magnetic insulators resulting in the flow of the magnon (spin) current. We take into account many-body magnon interactions and incorporate energy-dependent density of states of the magnetic insulators. Both features can strongly affect magnon distribution in the magnetic insulators and the coupling strengths between the leads and the dot, and thus, the thermally generated spin current. All the calculations are carried out in the weak coupling regime. We show, that results obtained with a density of states being a function of energy differ significantly from the ones obtained with a density of states taken as a constant. In turn, magnon interactions in the leads proved to be important at high temperatures and large values of energy of transported spin waves.
